Cloud-Edge Collaborative Large Models for Robust Photovoltaic Power Forecasting

Photovoltaic (PV) power forecasting in edge-enabled grids requires balancing forecasting accuracy, robustness under weather-driven distribution shifts, and strict latency constraints. Existing models work well under normal conditions but often struggle with rare ramp events and unexpected weather changes. Relying solely on cloud-based large models often leads to significant communication delays, which can hinder timely and efficient forecasting in practical grid environments. To address these issues, we propose a condition-adaptive cloud-edge collaborative framework *CAPE* for PV forecasting. *CAPE* consists of three main modules: a site-specific expert model for routine predictions, a lightweight edge-side model for enhanced local inference, and a cloud-based large retrieval model that provides relevant historical cases when needed. These modules are coordinated by a screening module that evaluates uncertainty, out-of-distribution risk, weather mutations, and model disagreement. Furthermore, we employ a Lyapunov-guided routing strategy to dynamically determine when to escalate inference to more powerful models under long-term system constraints. The final forecast is produced through adaptive fusion of the selected model outputs. Experiments on two real-world PV datasets demonstrate that *CAPE* achieves superior performance in terms of forecasting accuracy, robustness, routing quality, and system efficiency.

==> Chapter/c7_author.tex <==
\iffalse
%%============================================

\authorinfomation{Firstname1 Middlename1 Lastname1}{Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx}

\authorinfomation{Firstname2 Middlename2 Lastname2}{Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx}

\authorinfomation{Firstname3 Middlename3 Lastname3}{Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx}

\authorinfomation{Firstname4 Middlename4 Lastname4}{Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx}

\authorinfomation{Firstname5 Middlename5 Lastname5}{Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx}

\authorinfomation{Firstname6 Middlename6 Lastname6}{Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx}

\authorinfomation{Firstname7 Middlename7 Lastname7}{Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx Xxxx xxx xxx xxxx xxx}

\fi
%%@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@
%\vspace{-2em}
%% 隐藏作者信息（如需展示，请注释掉 \iffalse 与最后的 \fi ）

\authorinfo{photo}%
{Firstname1 Middlename1 Lastname1}%
{With a frequency range of approximately 70--300 MHz, the MWA spans a number of Earth and space-based broadcast bands, including the ubiquitous FM band (approximately 88--108 MHz in Australia), constituting a primary source of RFI at the MRO.  Likewise, the frequency range for SKA\_low is 50--350 MHz, also encompassing the FM band. With a frequency range of approximately 70--300 MHz, the MWA spans a number of Earth and space-based broadcast bands.}%
{xxxxxxxx@xxx.xxx.xx}

\authorinfo{photo}%
{Firstname2 Middlename2 Lastname2}%
{With a frequency range of approximately 70--300 MHz, the MWA spans a number of Earth and space-based broadcast bands, including the ubiquitous FM band (approximately 88--108 MHz in Australia), constituting a primary source of RFI at the MRO.  Likewise, the frequency range for SKA\_low is 50--350 MHz, also encompassing the FM band. With a frequency range of approximately 70--300 MHz, the MWA spans a number of Earth and space-based broadcast bands. With a frequency range of approximately 70--300 MHz, the MWA spans a number of Earth and space-based broadcast bands, including the ubiquitous FM band (approximately 88--108 MHz in Australia), constituting a primary source of RFI at the MRO.  Likewise, the frequency range for SKA\_low is 50--350 MHz, also encompassing the FM band. With a frequency range of approximately 70--300 MHz, the MWA spans a number of Earth and space-based broadcast bands.}%
{xxxxxxxx@xxx.xxx.xx}

\authorinfo{photo}%
{Firstname3 Middlename3 Lastname3}%
{Xxxx xxx xxx xxx xxxxxxxx xxxxxxxxx xxxxxxxx xxxxx xxxxxxxx xxxx xxxxxxxx xxxxx xxxxx xxxxxxxx xxxxx xxxxx xxxxxxxx xxxxx xxxxx xxxxxxxx xxxxx xxxxx xxxxxxxx xxxxx xxxxx xxxxxxxx xxxxx xxxxxxxx xxxxxxxx xxxxx xxxxx xxxxxxxx xxxxx xxxxx xxxxxxxx xxxxx xxxxx xxxxxxxx xxxxx xxxxxx xxxxxxxx xxx}%
{xxxxxxxx@xxx.xxx.xx}

\authorinfo{photo}%
{Firstname4 Middlename4 Lastname4}%
{Xxxx xxx xxx xxx xxxxxxxx xxxxxxxxx xxxxxxxx xxxxx xxxxxxxx xxxxxxxx xxxxxxxx xxx}%
{xxxxxxxx@xxx.xxx.xx}

%\begin{emsbiography}{photo}{Fei Zhang}
%    received the B.S. degree in electronic science and technology from Beijing University of Posts and Telecommunications (BUPT) in 2017. He is currently working towards the master degree in School of Electronic Engineering, BUPT. His current research is signal processing technology for wireless communications.
%\end{emsbiography}

%% 隐藏作者信息
